Learning Coordinated Bimanual Manipulation Policies using State Diffusion and Inverse Dynamics Models

When performing tasks like laundry, humans naturally coordinate both hands to manipulate objects and anticipate how their actions will change the state of the clothes. However, achieving such coordination in robotics remains challenging due to the need to model object movement, predict future states, and generate precise bimanual actions. In this work, we address these challenges by infusing the predictive nature of human manipulation strategies into robot imitation learning. Specifically, we disentangle task-related state transitions from agent-specific inverse dynamics modeling to enable effective bimanual coordination. Using a demonstration dataset, we train a diffusion model to predict future states given historical observations, envisioning how the scene evolves. Then, we use an inverse dynamics model to compute robot actions that achieve the predicted states. Our key insight is that modeling object movement can help learning policies for bimanual coordination manipulation tasks. Evaluating our framework across diverse simulation and real-world manipulation setups, including multimodal goal configurations, bimanual manipulation, deformable objects, and multi-object setups, we find that it consistently outperforms state-of-the-art state-to-action mapping policies. Our method demonstrates a remarkable capacity to navigate multimodal goal configurations and action distributions, maintain stability across different control modes, and synthesize a broader range of behaviors than those present in the demonstration dataset.

==> Sections/06-Limitations.tex <==
\section{Limitations}

Our work encompasses the following limitations. First, in the real-world Push-L task, our current policy requires the preliminary calculation of block positions using data from four RGBD cameras, which introduces time delays. Second, our method takes longer to train than the diffusion policy~\cite{Chi2023DiffusionPV} because the state space is typically larger than the action space, making the training longer. Third, collecting real-world demonstrations is time-consuming and labor-intensive.








%Second, our framework has not been evaluated against benchmarks that more accurately reflect real-world scenarios such as \cite{chen2023predicting}. The limitation may impede its scalability and applicability in broader and more complex environments.






